The unsteady overtopping of barriers by gravity currents and dam-break flows

The collision of a gravitationally-driven horizontal current with a barrier following release from a confining lock is investigated using a shallow water model of the motion, together with a sophisticated boundary condition capturing the local interaction. The boundary condition permits several overtopping modes: supercritical, subcritical, and blocked flow. The model is analysed both mathematically and numerically to reveal aspects of the unsteady motion and to compute the proportion of the fluid trapped upstream of the barrier. Several problems are treated. Firstly, the idealised problem of a uniform incident current is analysed to classify the unsteady dynamical regimes. Then, the extreme regimes of a very close or distant barrier are tackled, showing the progression of the interaction through the overtopping modes. Next, the trapped volume of fluid at late times is investigated numerically, demonstrating regimes in which the volume is determined purely by volumetric considerations, and others where transient inertial effects are significant. For a Boussinesq gravity current, even when the volume of the confined region behind the barrier is equal to the fluid volume, $30\%$ of the fluid escapes the domain, and a confined volume $3$ times larger is required for the overtopped volume to be negligible. For a subaerial dam-break flow, the proportion that escapes is in excess of $60\%$ when the confined volume equals the fluid volume, and a barrier as tall as the initial release is required for negligible overtopping. Finally, we compare our predictions to experiments, showing a good agreement across a range of parameters.

==> Sections/BackMatterJFM.tex <==
\backsection[Funding]{This work was supported by the EPSRC (E.W.G.S, grant number \href{https://gow.epsrc.ukri.org/NGBOViewGrant.aspx?GrantRef=EP/M506473/1}{EP/M506473/1}).}

\backsection[Declaration of interests]{The authors report no conflict of interest.}

\backsection[Author ORCID]{E.W.G. Skevington, \url{https://orcid.org/0000-0002-7709-9673}; A.J. Hogg, \url{https://orcid.org/0000-0002-9387-6698}.}

==> Sections/FrontMatterJFM.tex <==
\title{The unsteady overtopping of barriers by gravity currents and dam-break flows}
\shorttitle{Overtopping of barriers}

\author{Edward W.G. Skevington\aff{1,2}\corresp{\email{e.w.skevington@hull.ac.uk}}
 \and Andrew J. Hogg\aff{2}}
\shortauthor{E.W.G. Skevington and A.J. Hogg}
\affiliation{
	\aff{1} Energy and Environment Institute, University of Hull, HU6 7RX, England
	\aff{2} School of Mathematics, Fry Building, Woodland Road, Bristol, BS8 1UG, England
}

\maketitle

\begin{abstract}
	The collision of a gravitationally-driven horizontal current with a  barrier following release from a confining lock is investigated using a shallow water model of the motion, together with a sophisticated boundary condition capturing the local interaction. The boundary condition permits several overtopping modes: supercritical, subcritical, and blocked flow. The model is analysed both mathematically and numerically to reveal aspects of the unsteady motion and to compute the proportion of the fluid trapped upstream of the barrier. Several problems are treated. Firstly, the idealised problem of a uniform incident current is analysed to classify the unsteady dynamical regimes. Then, the extreme regimes of a very close or distant barrier are tackled, showing the progression of the interaction through the overtopping modes. Next, the trapped volume of fluid at late times is investigated numerically, demonstrating regimes in which the volume is determined purely by volumetric considerations, and others where transient inertial effects are significant. For a Boussinesq gravity current, even when the volume of the confined region behind the barrier is equal to the fluid volume, $30\%$ of the fluid escapes the domain, and a confined volume $3$ times larger is required for the overtopped volume to be negligible. For a subaerial dam-break flow, the proportion that escapes is in excess of $60\%$ when the confined volume equals the fluid volume, and a barrier as tall as the initial release is required for negligible overtopping. Finally, we compare our predictions to experiments, showing a good agreement across a range of parameters.
\end{abstract}

==> Sections/Step/SteepSlope.tex <==
\section{Asymptotic behaviour on a steep slope} \label{sec:overtop_slopeshock}

\andy{Should this be a separate short paper?}

We next investigate the behaviour of fluid on a slope given by \cref{eqn:very_steep_slope} as $\epsilon \rightarrow 0$. The timescale of evolution on the slope will be much faster than that of the interior thus, as long as we are not at the instant at which a shock collides with the slope, the dynamics on the slope are quasi-static and obey
\begin{align}
	\dv{x} \qty(uh) &= 0 &
	\dv{x} \qty(u^2 h) + h \dv{x}(h+b) = 0.
\end{align}
These equations admit continuous solutions where $q$ and $E$ are constant, where
\begin{align}
	q &\eqdef uh	&
	E &\eqdef \frac{u^2}{2} + h + b
\end{align}
are the volume flux and energy respectively. Indeed, if $q=0$ then the only solution is constant surface elevation $h + b$. Otherwise there exists discontinuous solutions to the system, representing steady shocks on the slope. Continuous solutions which are not critical at the top clearly stable (any perturbations advected off the slope in time $\order{\epsilon^{-1}}$), it is possible to construct steady states which are critical at the top and these will be considered later. For the case of shocks it is not so clear, as the shock itself may be advected out of the domain leaving the solution on the slope continuous. For a perturbation of size $\order{\delta}$ the dynamics in the continuous regions to either side of the shock will evolve on a timescale $\order{\epsilon^{-1}}$, whereas the shock may exit the slope over time $\order{\flatfrac{\delta}{\epsilon}}$. For this reason we investigate the stability of a steady state solution involving a shock on a slope by considering the solution on either side of the shock to be steady. To simplify the analysis we will work in a frame where the fluid is retreating across the slope ($q<0$) but the slope may be either up or down ($B \in \mathbb{R} \setminus \{0\}$). To achieve this from our problem formulation it may be necessary to change variables $x \rightarrow -x$, $u \rightarrow -u$.

\subsection{Stability of shocks on slopes}

In our investigation of the stability of shocks on slopes we use the notation $q_-$, $E_-$ to denote the flux and energy of the fluid to the left of the shock, and $q_+$, $E_+$ to the right ($E_- < E_+$), along with $u_{\pm}$ and $h_{\pm}$ to denote the velocity and depth immediately adjacent to the shock. The bed elevation at the shock is denoted $b_s$. Given the states to either side it is possible to determine the steady state location of the shock. The location of the shock does not effect the state to the right as this is supercritical, and to the left at location $x=L$ the value of $\alpha=\alpha_L$ is determined by the imposed steady state, however $\beta = \beta_L$ is determined by the shock conditions, and in this way $q_-$, $E_-$ vary as the shock moves. The value of $\beta_L$ and the shock speed $s$ are determined by the shock conditions given $b_s$.

We expand all variables around the steady state, that is
\begin{subequations}\begin{align}
	q_{\pm} &= q_{0} 	 + \delta q_{\pm 1} + \lorder{\delta},	&
	E_{\pm} &= E_{\pm 0} + \delta E_{\pm 1} + \lorder{\delta},	\\
	u_{\pm} &= u_{\pm 0} + \delta u_{\pm 1} + \lorder{\delta},	&
	h_{\pm} &= h_{\pm 0} + \delta h_{\pm 1} + \lorder{\delta},	\\
	b_s     &= b_0       + \delta b_1       + \lorder{\delta},	&
	s       &= 0		 + \delta s_1       + \lorder{\delta}.							
\end{align}\end{subequations}
The first task is to find expressions for $E_{\pm 1}$, $q_{\pm 1}$. To the right of the shock we have $E_{+ 1}=q_{+ 1}=0$ by our earlier discussion. To the left of the shock the value of $\alpha_L$ is known, but the other values at $x=L$ may be perturbed from there steady state values, that is
\begin{align}
	u_{L} 		&= u_{L 0} 		+ \delta u_{L 1} 		+ \lorder{\delta},	&
	h_{L} 		&= h_{L 0} 		+ \delta h_{L 1} 		+ \lorder{\delta},	&
	\beta_{L} 	&= \beta_{L 0} 	+ \delta \beta_{L 1} 	+ \lorder{\delta}.
\end{align}
Expanding the expressions for $\alpha_L$ and $\beta_L$ in terms of $u_L$ and $h_L$ and rearranging we find
\begin{subequations}\begin{align}
	u_{L 1} &= \frac{\beta_{L 1}}{2},	&
	h_{L 1} &= - \sqrt{h_{L0}} \frac{\beta_{L 1}}{2},
\intertext{thus, expanding the expressions for energy and flux,}
	E_{- 1} &= \frac{\lambda_{\beta L 0} \beta_{L 1}}{2},	&
	q_{- 1} &= - \sqrt{h_{L0}}\frac{\lambda_{\beta L 0} \beta_{L 1}}{2},
\end{align}\end{subequations}
where $\lambda_{\beta L 0} = u_{L0}-\sqrt{h_{L0}}$. Now we have expressions for $E_{\pm 1}$, $q_{\pm 1}$ we make use of the shock conditions, derived in \cref{sec:overtop_PerturbShock},

\sidebysidesubequations{eqn:SW_shock_con_ptb_slope}
{s_1 = \flatfrac{\shock*{q_1}}{\shock*{h_0}},}{eqn:SW_shock_con_slope_ptb_speed}
{and}
{0 = \shock*{ h_{0} \qty(E_{1} - b_1) + u_{0} q_{1}}.}{eqn:SW_shock_con_slope_ptb_restrict}
Substituting into \cref{eqn:SW_shock_con_slope_ptb_restrict} yields
\begin{subequations}\begin{align}
	\frac{\lambda_{\beta L 0} \beta_{L 1}}{2} &= -\frac{\shock*{h_0}}{\sqrt{h_{L 0}}} K b_1 
	&\textrm{where}&&
	K &= \qty( - u_{- 0} + \frac{h_{- 0}}{\sqrt{h_{L 0}}} )^{-1} > 0,
\end{align}
and subsequently substituting into \cref{eqn:SW_shock_con_slope_ptb_speed} yields
\begin{align}
	s_1 &= - K b_1.
\end{align}\end{subequations}
We can now proceed to finding the trajectory of the shock location $x_s$. We suppose that local to the equilibrium steady state at which $x_s = x_0$, $b$ can be expanded as
\begin{align}
	b &= b_0 + \tilde{b}_1 \qty(\frac{x-x_0}{\epsilon})^p + \lorder{\delta},
\end{align}
$p>0$, thus we transform as
\begin{align}
	x_s &= x_0 + \epsilon \delta^{1/p} \tilde{x}(\tilde{t}) &
	t   &= \epsilon \delta^{(1/p)-1} \tilde{t}
\end{align}
and $b_1 = \tilde{b}_1 \tilde{x}^p$, $s_1 = \dv*{\tilde{x}}{\tilde{t}}$,
\begin{equation}
	\dv{\tilde{x}}{\tilde{t}} = - K \tilde{b}_1 \tilde{x}^p
\end{equation}
which has solutions
\begin{equation}\begin{multicasesd}[3]
	\tilde{x} &= \exp\qty( -K \tilde{b}_1 (\tilde{t} - \tilde{t}_0) )	&
	\textrm{for}&&
	p &= 1,
	\\
	\tilde{x} &= \qty( (p-1) K \tilde{b}_1 (\tilde{t} - \tilde{t}_0)  )^{-1/(p-1)}	&
	\textrm{for}&&
	p &\neq 1,
\end{multicasesd}\end{equation}
where $\tilde{t}_0$ is a constant. For the slope \cref{eqn:very_steep_slope}, on $L < x_0 < L+\epsilon$ we have $p=1$ and $\tilde{b}_1 B >0$, thus the dynamics are stable for $B>0$. At $x_0 = L$, $\hat{x}>0$ we have $p=2$ and $\tilde{b_1} B > 0$, thus the dynamics are stable for $B>0$. At $x_0 = L + \epsilon$, $\hat{x}<0$ we have $p=2$ and $\tilde{b_1} B < 0$, thus the dynamics are stable for $B>0$.  At $x_0 = L$, $\hat{x}<0$ and $x_0 = L+\epsilon$, $\hat{x}<0$ any perturbation to the left and right states of $\order{\delta}$ will produce a constant speed of the same order, thus the equilibrium is neutrally stable. Thus we deduce that the condition for stability is
\begin{equation}
	q B < 0,
\end{equation}
that is the fluid flows down hill.

\subsection{Stability of critical continuous solutions}

We next consider a continuous flow that is critical at the top, that is the unperturbed state has energy $E_0$ and flux $q_0$ where
\begin{equation}
	E_0 = \frac{3}{2}q_0^{\flatfrac{2}{3}} + B,
\end{equation}
and we take $B>0$ and $q_0$ of either sign. There are four possible flow configurations for this, corresponding to subcritical/supercritical flow up/down the slope (note that whilst flow at the top is critical, anywhere else on the slope the flow has energy which exceeds the critical energy, and we classify subcritical/supercritical based on the behaviour away from the top). We are interested in the stability with respect to changing the upstream and down stream states. To do this we expand the solution local to the crest of the slope, that is we impose a new coordinate system $\tilde{x}$ where $x = L + \epsilon \qty(1 + \delta \tilde{x} )$ for $0 < \delta \ll 1$. The value of $\delta$ is chosen to be the magnitude of the applied perturbation. In this coordinate system
\begin{align}
	b &= B(1 - \delta^2 2 \tilde{x}^2)
	&&\textrm{for}&
	\tilde{x} &\leq 0,
	&&\textrm{and}&
	b &= B
	&&\textrm{for}&
	\tilde{x} &\geq 0.
\end{align}
Expanding $u$ and $h$ in the region $\tilde{x}<0$ yields the expressions
\begin{subequations}\begin{align}
	h &= q_0^{2/3} + \delta \qty( -s 2 q_0^{1/3} \sqrt{\frac{B}{3}} \tilde{x} + h_1(x,t) ) + \order{\delta^2}
	\\
	u &= q_0^{1/3} + \delta \qty( s 2 \sqrt{\frac{B}{3}} \tilde{x} + u_1(x,t) ) + \order{\delta^2}
\end{align}\end{subequations}
where $s=\sign(q_0)$ for supercritical flow and $s=-\sign(q_0)$ for subcritical flow, and $h_1$, $u_1$ are the perturbations. When $q_0>0$ the $\alpha$-characteristics are moving fast and the $\beta$-characteristics are moving slow, that is $\lambda_\alpha = \order{1}$, $\lambda_\beta = \order{\delta}$, and when $q_0<0$ the $\beta$-characteristics are moving fast and the $\alpha$-characteristics are moving slow. We introduce the timescale $\tilde{t} = t/\epsilon$ so that $\dv*{\tilde{x}}{\tilde{t}}$ is $\order{1}$ for the slow family. Substituting our expansions into \eqref{eqn:SW_characteristics_bed_alpha} for $q_0>0$ and \eqref{eqn:SW_characteristics_bed_beta} for $q_0<0$ we get the equation for the fast family at leading order as
\begin{subequations}
\begin{align}
	\pdv{x} \qty( u_1 + \frac{h_1}{q_0^{1/3}} ) &= 0
	&&\therefore&
	u_1 + \frac{h_1}{q_0^{1/3}} = U_1(\tilde{t}),
\end{align}
where $U_1$ is a perturbation in the value of the fast moving family of characteristics, which in this time scale causes an instantaneous change. Substituting our expansions into \eqref{eqn:SW_characteristics_bed_beta} for $q_0>0$ and \eqref{eqn:SW_characteristics_bed_alpha} for $q_0<0$ we get the equation for the slow family at leading order as
\begin{align}
	\dv{\tilde{t}}\qty( \Lambda - \frac{U_1}{4} ) &= k^2 \tilde{x}
	&&\textrm{on}&
	\dv{\tilde{x}}{\tilde{t}} &= \Lambda \eqdef \frac{3}{2} u_1 - \frac{1}{2} U_1 + s k \tilde{x}
\end{align}
where $k = \sqrt{3B}$. If $U_1$ is discontinuous in time then $\Lambda - U_1/4$ must be continuous, whilst if $U_1$ is constant then
\begin{align} \label{eqn:asyp_char_top_soln}
	\Lambda 	&= C s k e^{s k \tilde{t}} - D s k e^{-s k \tilde{t}}
	&
	\tilde{x}   &= C e^{s k \tilde{t}} + D e^{-s k \tilde{t}}
\end{align}
\end{subequations}
where $C$ and $D$ are constants along each slow characteristic curve, and we will treat them as functions of $\tilde{x}_0$, the value of $\tilde{x}$ when $\tilde{t} = 0$, that is $C(\tilde{x}_0) + D(\tilde{x}_0) = \tilde{x}_0$. For time $\tilde{t}<0$ there is no perturbation, $u_1 = U_1 = 0$ thus $\Lambda = s k \tilde{x}$. This implies $D=0$ thus $C = \tilde{x}_0$ and the characteristics are $\tilde{x} = x_0 e^{s k \tilde{t}}$. At time $\tilde{t}=0$ we perturb the states outside the slope and $U_1$ takes a non-zero value, thus for the characteristics close to the top $C$ and $D$ change discontinuously to $C = \tilde{x_0} - s \flatfrac{U_1}{8k}$ and $D = s \flatfrac{U_1}{8k}$, thus
\begin{align}
	\tilde{x} &= \tilde{x}_0 e^{skt} + \frac{U_1}{4k} \sinh{kt}.
\end{align}

For $s=1$ the unperturbed slow characteristics diverge from the top of the slope exponentially. Perturbing with $U_1 > 0$  then the characteristic with $x_0 = -U_1/8k$ tends to the top, whilst those with $x_0 < -U_1/8k$ continue to have the same behaviour as previously, and with $x_0 > -U_1/8k$ escaping the slope. Thus the flow remains critical at the top. With $U_1 < 0$ causes the originally critical characteristic at the top to travel down the slope, thus the flow is of the same type but now the energy at the top is greater than the critical energy. Thus the dynamics are stable to perturbing $U_1$ for supercritical flow down a slope ($q_0<0$) and subcritical flow up a slope ($q_0>0$).

For $s=-1$ the unperturbed characteristics converge on the top of the slope. Perturbing with $U_1 > 0$ the characteristics all climb the slope faster, thus this is flow of the same type but the energy at the top is greater than the critical energy. With $U_1<0$ the region at the crest has characteristics moving down the slope, which necessarily collide with the characteristics moving up the slope from the bottom. This creates a shock, and the stability dependent on the stability of the shock. Thus with respect to perturbing $U_1$ supercritical flow up a slope ($q_0>0$) is unstable, whilst subcritical flow down a slope ($q_0<0$) is stable.

The discussion so far has been with regard to perturbing the fast characteristic family, but it is also possible to perturb the slow characteristic family. These characteristics will have the form \cref{eqn:asyp_char_top_soln} once they are close to the top of the slope $\tilde{x}<0$. With $s=1$ the only possibility is to have leftward moving characteristics entering from $\tilde{x} = 0$ which results in flow of the same type but energy at the crest is greater than the critical energy. The same happens with $s=-1$ and the characteristics are moving up the slope faster than in the unperturbed state. If the characteristics are moving up the slope slower then they necessarily turn around and move back down the slope intersecting with those moving up, which creates a shock, whose stability is as previously. Thus the stability with respect to perturbing the slow moving family of characteristics is the same as with respect to the fast moving.

We conclude then that, if the energy at the top is critical, supercritical flow up a slope is unstable whilst all other states are stable. This is why the supercritical overtopping boundary condition was stated as a strict inequality in \cref{sec:overtop_PF}.

\subsection{Shock on slope as a shock condition}

\begin{figure}
	\centering
	\includegraphics{Overtopping_Analytics/ShockSlope_Energy.pdf}
	\caption{Plot showing the permitted energetic states on a steep slope \cref{eqn:very_steep_slope} when $q<0$ and $B>0$. The solid curves indicate permitted states, as does the shaded region. The dash dot cures are used for the construction, but are not permitted states. All of the curves are labelled with the condition used to plot them, in particular where a value of $b_s$ is given this is a solution to \cref{eqn:SW_shock_con_slope} with the value of $b_s$ given For this plot we denote the value of the bed elevation to the left of the steep slope by $b_-$ and the value to the right by $b_+$, this figure is plotted for $b_- = 0$ and $b_+ = B = q^{2/3}$, and the critical energy is $E_c = 3 q^{2/3} / 2$.}
	\label{fig:ShockSlope_Energy}
\end{figure}

From here on we take $q < 0$ and $B > 0$. In the limit $\epsilon \rightarrow 0$ the dynamics on a steep slope can be understood on the large scale ($x-L = \order{1}$) as creating a discontinuity, for which we impose some condition. The conservation of mass gives $\shock*{q}=0$. When the dynamics on the slope are continuous on the small scale ($x-L = \order{\epsilon}$) they are energy conserving, thus the large scale condition is $\shock*{E} = 0$. Otherwise on the small scale, the dynamics are discontinuous. Defining $\tilde{E}_{\pm} = \flatfrac{E_{\pm}}{q^{2/3}}$, $\tilde{h}_{\pm} = \flatfrac{h_{\pm}}{q^{2/3}}$, $\tilde{b}_s = \flatfrac{b_s}{q^{2/3}}$ the discontinuous states are defined implicitly by
\begin{align}	\label{eqn:SW_shock_con_slope}
	\tilde{E}_{\pm} &= \frac{1}{2 \tilde{h}_{\pm}^2} + \tilde{h}_{\pm} + \tilde{b}_s, &
	\shock*{\frac{1}{\tilde{h}} + \frac{\tilde{h}^2}{2}} &= 0.
\end{align}
where $\tilde{h}_- > 1 > \tilde{h}_+ > 0$. We aim to find the region in the $(\tilde{E}_-,\tilde{E}_+)$ plane that is accessible by a shock given a value of the flux $q$. The permitted shocks may be parametrised by $\tilde{h}_+$, each permitted value of $\tilde{h}_+$ having a unique corresponding $\tilde{h}_-$, and defining a curve in the $(\tilde{E}_- - \tilde{b}_s,\tilde{E}_+ - \tilde{b}_s)$ plane. The accessible region in the $(\tilde{E}_-,\tilde{E}_+)$ plane is found by translating this curve which sweeps out an area, thus is bound by the curves for $\tilde{b}_s=0$ and $\tilde{b}_s = \flatfrac{B}{q^{2/3}}$. Not all energies found in this manner are permissible, because the energy to the right of the shock must be sufficient for the energy at the top of the slope to be at least critical, that is $\tilde{E}_+ \geq 3/2 + \flatfrac{B}{q^{2/3}}$. This defines the accessible region, which is shown in \cref{fig:ShockSlope_Energy}.

\subsection{Discussion}

We have found that, for fluid flowing up a slope, energy is conserved. This was assumed in the problem formulation for flow over a barrier and justifies its use there. Moreover for the slope case, the supercritical Froude number condition implies that the flow at the top of the slope will be supercritical at the instant of collision, and consequently \emph{the dynamics at collision will be the same as for the barrier}.

Conversely, for fluid flowing down a slope, it is possible for a shock to be sustained on the slope. This is important for our problem as it is a behaviour we expect to see. The inertia of the fluid front when it collides with the slope will (for a sufficiently short barrier) drive some volume of fluid up the slope. Once this initial phase has passed and the fluid at the bottom of the slope has become subcritical then, provided the depth of fluid at the bottom of the slope is less than the height of the slope, the fluid at the top of the barrier is able to critically backflow. That is to say, at $x=L+\epsilon$ we will have $u = -\sqrt{h}$, which is the behaviour discussed in \note{cite my paper}. This necessitates a shock on the slope. The backflow of fluid from the region $x > L$ is the crucial difference between the barrier and the slope. The other difference is the possibility of subcritical flow at the top of the slope, that is at $x = L+\epsilon$ we have $0 < u < \sqrt{h}$, meaning the flow up the slope is not controlled by energy balance with a critical state, though we expect this behaviour to be rare and of little consequence.

==> Sections/Step/VolumeOutStep.tex <==
\section{Numerical evaluation of fluid outflow over a slope}

\begin{figure}
	\centering
	\includegraphics{Overtopping_Numerics_Metrics/VolOut_Step.pdf}
	\includegraphics{Overtopping_Numerics_Metrics/VolOut_Step_Diff.pdf}
	\caption{(a) The volume of fluid that has overtopped the obstacle at large times for the barrier, the black lines are contours of constant volume. (b) The net difference in volume of fluid that has overtopped the obstacle for the barrier and slope (barrier minus slope). In both figures we plot in a white dashed line $B=1$, and in a white solid line the the maximum $B$ for overtopping from \cref{fig:InfWall_MaxDepth}.}
	\label{fig:OutflowVolume_Step}
\end{figure}

We investigate numerically the dynamics produced by a lock release into a slope, in the same manner as was used for lock release into a barrier in \cref{sec:overtop_slopeshock}. From the discussion in \cref{sec:overtop_slopeshock} we know that, at the instant of collision, the dynamics for the slope are the same as for the barrier (provided $\Fro \geq 1$), and so the same initial behaviour will be same until outflow ceases. This means that the maximal obstacle height for outflow plotted in \cref{fig:InfWall_MaxDepth} is the same. Once outflow ceases, the fluid on $x>L$ will locally reverse its flow direction and pour back down the slope. The flow at the top of the slope will be critical, and will accelerate supercritically down the steep slope until a shock on the slope, at which point there is a transition to subcritical flow which continues down into the basin $x<L$. For values of $\Fro$, $L$ and $B$ we may see a secondary overtopping when a shock collides with the slope and deepens the fluid there sufficiently.

To enable a direct comparison with the barrier case we simulate for $\Fro = \sqrt{2}$, and employ the measure of outflow $\Delta V$ as previously, see \cref{eqn:escaped_volume}, extending the integral up to $L+\epsilon$ for our slope of finite width \cref{eqn:very_steep_slope}. In \cref{fig:OutflowVolume_Step} we plot $\Delta V$ for the case of the slope using the same format as \cref{fig:OutflowVolume_Crit}. The overtopped volume is very similar for our two types of obstacle, and the additional overtopped volume for the barrier as compared to the slope is shown in \cref{fig:OutflowVolume_Step}(b). For $BL \lesssim 1/3$ there is little difference as both obstacle types produce the minimum overtopping of $\Delta V \approx 1-BL$, and for $BL \gtrsim 2$ there is insufficient inertia so $\Delta V \approx 0$. Between these two extremes there is sufficient inertia to overtop in excess of what is required by volume conservation, a portion of this then undergoes backflow, giving a net reduction in overtopping of up to $0.13$ for the slope.

==> Sections/VolumeOutParticles.tex <==
\section{Particle driven currents}	\label{sec:overtop_particle}

\subsection{Problem formulation}

We now analyse a gravity current driven by a suspended particle load. We operate under the same assumptions that were utilised in \cref{sec:overtop_PF}, except that now the density of the current can change with the volume concentration of particles, and the interstitial fluid is assumed to be the same density to the ambient. We further assume that the current is Boussinesq, that is the net density of the particle suspension is only slightly larger than the density of the ambient, the bed is not erodible, there is no reworking of settled particles, and the settled particles have a negligible effect on the topography. Thus the governing equations are
\begin{subequations}\label{eqn:ot:SWP_sys}\begin{align}
	\pdv{h}{t} + \pdv{}{x} (uh) &= 0,	\\
	\pdv{}{t} (uh) + \pdv{}{x} \ppar*{ h u^2 + \phi \frac{h^2}{2} } &= -\phi h \dv{b}{x},	\\
	\pdv{}{t} (\phi h) + \pdv{}{x} ( u \phi h ) &= - v_s \phi,	\\
	\pdv{\psi}{t} &= v_s \phi.
\end{align}\end{subequations}
We have non-dimensionalised the particle concentration $\phi(x,t)$ by the initial uniform concentration $\Phi$, the deposited load $\psi(x,t)$ by $\Phi Z$, the settling velocity $v_s$ by $Z \sqrt{g' Z}/X$, and all other variables using the same scales as in \cref{sec:overtop_PF} with $g' = g_p' \Phi$ where $g_p' \eqdef \frac*{g (\rho_p - \rho_a)}{\rho_a}>0$ is the reduced gravity of the particles, and $\rho_p$ is the density of particles.

As before the domain is $0 \leq x \leq x_f(t)$, and the initial conditions are $h(x,0)=\phi(x,0)=1$, $u(x,0)=\psi(x,0)=0$, $x_f(0)=1$. The bed is horizontal up until the obstacle at $x=L \geq 1$, that is $b(x) = 0$ for $0 \leq x < L$, and the fluid is confined to the rear by an insurmountable back wall imposing $u(0,t)=0$. The motion during $t>0$ is due to the removal of the lock at $x=1$ which produces a moving front obeying the condition at $x=x_f$
\begin{equation}
	\dv{x_f}{t} = u = \Fro \sqrt{\phi h}
\end{equation}

To model the barrier we exploit the fact that the barrier has a small horizontal extent, thus settling can be neglected and $\phi$ is constant up the incline in the quasi-static dynamics. From this we deduce that the correct measure of the energy change between the base and crest of the barrier is 
\begin{equation}
	\Delta E_w \eqdef \Delta E (u_w/\sqrt{\phi_w} , h_w , B).
\end{equation}
Supercritical overtopping occurs when $u_w > \sqrt{\phi_w h_w}$, $\Delta E_w > 0$; subcritical overtopping requires $\Delta E_w = 0$ and $0 \leq u_w \leq \sqrt{\phi_w h_w}$; and no outflow requires $q_w = 0$ and $\Delta E_w < 0$.

We observe that the problem formulated here, whilst modelling a slightly different physical problem, is mathematically a generalisation of the problem in \cref{sec:overtop_PF}, and our earlier problem is recovered in the case $v_s = 0$. This allows us to utilise many of our earlier results for the case $v_s>0$. In particular, over sufficiently short intervals of length and time the effect of settling is negligible, thus the results of the boundary Riemann problem \cref{sec:overtop_close} still apply, using that in the solution $\phi$ is constant to construct the rescaled variables
\begin{align}
	\hat{x} &= \frac{x-L}{\delta},
	&
	\hat{t} &= \sqrt{\phi B} \frac{t - t_0}{\delta},
	&
	\hat{u} &= \frac{u}{\sqrt{\phi B}},
	&
	\hat{h} &= \frac{h}{B}.
\end{align}

\subsection{Numerical evaluation of outflow for a particle laden current}

To simulate our system of equations, we utilise the Boussinesq assumption to set $\Fro = \sqrt{2}$. To determine an appropriate $v_s$ we utilise the run out length, that is the distance over which the vast majority of particles have settled out. The method outlined in \citet[\S 9.1.8]{bk_Ungarish_GCI} yields the expression
\begin{equation}
	L_\infty = \ppar*{1 + \frac{5 \Fro}{v_s}}^{2/5}.
\end{equation}
If $L_\infty-1 \ll 1$ then all the particles immediately fall out, which is not an interesting case, whilst if  $L_\infty \gg 1$ then, to leading order, we are in the constant density regime discussed previously. We choose $v_s = 0.05$ which yields $L_\infty = 7.3$, thus we operate in the regime where settling and the interaction with the barrier occur on the same timescale.

We simulate our system over $L \in \{1 , 1.5 , \ldots , 10\}$ and $BL \in \{0 , 0.2 , \ldots , 3\}$ at a resolution of 1000 cells. We employ the measure
\begin{align}\label{eqn:ot:escaped_particles}
	\Delta P &= 1 - P_\infty,
	&&\textrm{where}&
	P_\infty &= \lim_{t \rightarrow \infty} \int_{0}^L \phi h + \psi \dd{x}
\end{align}
which measures the portion of the particle load which has escaped over the barrier. This is approximated numerically by simulating until 
\begin{equation}
	\int_{0}^L \phi h \dd{x} = 0.001
\end{equation}
the particle load at this time being used to approximate $P_\infty$.

\begin{figure}
	\centering
	\includegraphics{Overtopping_Numerics_Metrics/VolOut_Crit_Par.pdf}
	\caption{The volume of fluid that has overtopped the obstacle at large times for a particle laden current with $\Fro = \sqrt{2}$, $v_s = 0.05$, the black lines are contours of constant volume.}
	\label{fig:ot:OutflowVolume_CritPar}
\end{figure}

The results are plotted in \cref{fig:ot:OutflowVolume_CritPar}, which is qualitatively different to the non-settling case in \cref{fig:ot:OutflowVolume_Crit}. During the initial phase where the dense fluid is spreading as a gravity current, the particle load is settling out, which has two effects. Firstly, there are fewer particles suspended in the current, thus even if a large volume of fluid overtops only a small portion of the particle load may accompany it. This explains why, at constant $BL$, the portion of overtopped particles is a decreasing function of $L$, whereas without settling the overtopped portion of particles is the same as the overtopped volume and is largely independent of $L$. Secondly, at collision a portion of the kinetic energy of the fluid is converted into potential energy, less some dissipation in the shock. Reducing the particle load does not reduce the kinetic energy (in the Boussinesq model), but it does mean that the height of the current for equivalent potential energy does increase, going as $h \propto 1/\phi$. Thus, at collision the fluid attains a much greater height and is able to overtop much taller barriers. This is why, as $L$ increases, the height of barrier required to reduce the overtopping gets progressively taller.

==> Templates/StandardMathsMacros.tex <==
%My macros for the math environment

\usepackage{xparse}
\makeatletter




%---BRACKETS----

%Normal brackets

\DeclarePairedDelimiter{\ppar}{\lparen}{\rparen}
\DeclarePairedDelimiter{\pang}{\langle}{\rangle}
\DeclarePairedDelimiter{\pbrc}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\pbrk}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\pgrp}{\lgroup}{\rgroup}

%Bracket-like structures

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\round}{\lfloor}{\rceil}

\DeclarePairedDelimiter{\eval@wdot}{.}{\rvert}
\NewDocumentCommand{\eval}{som}{%
	\IfBooleanTF{#1}
    	{\eval@wdot*{#3}}
   		{\IfNoValueTF{#2}{#3\rvert}{\eval@wdot[#2]{#3}}}%
}

\DeclarePairedDelimiterX{\setpred}[2]{\lbrace}{\rbrace}{\: #1 \: \delimsize\vert \: #2 \:}
\DeclarePairedDelimiter{\shock}{[}{]_{-}^{+}}




%---OPERATORS---

\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\minmod}{minmod}
\DeclareMathOperator{\diag}{diag}




%---DIMENSIONLESS CONSTANTS---
%Define carefully, some of these are defined in the JFM template

%\Rey Reynolds number 
\ifdefined\Rey\else
	\newcommand\Rey{\mbox{\textit{Re}}}
\fi

%\Pran Prandtl number
\ifdefined\Pran\else
	\newcommand\Pran{\mbox{\textit{Pr}}} 
\fi

%\Pen Peclet number
\ifdefined\Pen\else
	\newcommand\Pen{\mbox{\textit{Pe}}}
\fi

%\Fro Froude number
\ifdefined\Fro\else
	\newcommand\Fro{\mbox{\textit{Fr}}}
\fi

%\Ric Richardson number
\ifdefined\Ric\else
	\newcommand\Ric{\mbox{\textit{Ri}}}
\fi

%\Sch Richardson number
\ifdefined\Sch\else
	\newcommand\Sch{\mbox{\textit{Sc}}}
\fi



%---VECTOR---
\newcommand*\vecb[1]{\bm{#1}}
\newcommand*\vecbu[1]{\hat{\vecb{#1}}}
\newcommand*\dotp{\mathpalette\omitdummy@{0.5}}
\newcommand*\ddotp{\bm{:}}




%---CALCULUS---
%Uses the calculus syntax from the Physics package with a few modifications
%
%For fractions p/q, following applies
%\frac{p}{q}, standard
%\frac*{p}{q}, flat
%\frac**{p}{q}, flat, autosize slash
%\frac*[\size]{p}{q}, flat, slash size of \size
%
%For differential d syntax is
%\dd*[power]{measure}
%Star removes spacing
%
%For derivative df/dx, stars the same as for \frac, optional argument the order of the derivative
%\dv(frac syntax here)[order]{f}{x}
%If wanting to use a flat derivative without sizing with order, then \dv*[][n]{f}{x}
%
%For partial derivative df/dx, use \pdv with syntax as for \dv
%For mixed partial derivative d2f/dxdy, use \pdvt three arguments for f,x,y
%NOT IMPLEMENTED YET Alternatively, for d^n f/dx_1 ... dx_n use
%\pdvm(frac syntax here){n}{f}{x_1}...{x_n}

%\frac
\let\frac@nostar\frac
\DeclarePairedDelimiterX{\frac@starwdot}[2]{.}{.}{#1 \delimsize/ #2}
\NewDocumentCommand{\frac@star}{somm}{%
	\IfBooleanTF{#1}
    	{\frac@starwdot*{#3}{#4}}
    	{\IfNoValueTF{#2}{#3/#4}{\frac@starwdot[#2]{#3}{#4}}}%
}
\renewcommand*\frac{\@ifstar{\frac@star}{\frac@nostar}}

%\dd
\NewDocumentCommand{\dd}{som}{%
	\IfBooleanF{#1}{\,}%
	\IfNoValueTF{#2}{%Check whether optional argument is given
		\mathrm{d} #3%
	}{%
		\mathrm{d}^{#2} #3%
	}%
	\IfBooleanF{#1}{\,}%
}

%\dv
\NewDocumentCommand\dv@nostar{O{}mm}{%
	\frac@nostar{\mathrm{d}^{#1} #2}{{\mathrm{d} #3}^{#1}}
}
\NewDocumentCommand{\dv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\mathrm{d}^{#2} #4}{{\mathrm{d} #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\mathrm{d}^{#3} #4}{{\mathrm{d} #5}^{#3}}%
		\else
			\frac*[#2]{\mathrm{d}^{#3} #4}{{\mathrm{d} #5}^{#3}}%
		\fi
	}%
}
\newcommand*\dv{\@ifstar{\dv@star}{\dv@nostar}}

%\pdv
\NewDocumentCommand\pdv@nostar{O{}mm}{%
	\frac@nostar{\partial^{#1} #2}{{\partial #3}^{#1}}
}
\NewDocumentCommand{\pdv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^{#2} #4}{{\partial #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\else
			\frac*[#2]{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\fi
	}%
}
\newcommand*\pdv{\@ifstar{\pdv@star}{\pdv@nostar}}

%\pdvt
\NewDocumentCommand\pdvt@nostar{mmm}{%
	\frac@nostar{\partial^2 #1}{\partial #2 \partial #3}
}
\NewDocumentCommand{\pdvt@star}{sO{}mmm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^2 #3}{\partial #4 \partial #5}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\partial^2 #3}{\partial #4 \partial #5}%
		\else
			\frac*[#2]{\partial^2 #3}{\partial #4 \partial #5}%
		\fi
	}%
}
\newcommand*\pdvt{\@ifstar{\pdvt@star}{\pdvt@nostar}}



%%\pdvm
%\NewDocumentCommand\pdvm@nostar@two{mmmm}{%
%	\frac{\partial^2 #2}{\partial #3 \partial #4}
%}
%\NewDocumentCommand{\pdvm@star@two}{sO{}mmm}{%
%	|#1,#2,#3,#4,#5|
%%	\IfBooleanTF{#2}{%
%%		\frac**{\partial^2 #4}{\partial #5 \partial #6}%
%%	}{%
%%		\if \relax\detokenize{#3}\relax
%%			\frac*{\partial^2 #4}{\partial #5 \partial #6}%
%%		\else
%%			\frac*[#3]{\partial^2 #4}{\partial #5 \partial #6}%
%%		\fi
%%	}%
%}
%\newcommand*\pdvm@nostar[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm@STAR[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm{\@ifstar{\pdvm@star}{\pdvm@nostar}}

%\def\pdvm@str@frac{frac}
%\def\pdvm@str@flat{flat}
%\def\pdvm@str@slsh{slsh}
%
%\NewDocumentCommand{\pdvm@two}{mmmmm}{
%	F|#1,#2,#3,#4,#5|
%}
%
%\newcommand*\pdvm@nostar[1]{%
%	A|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@frac}{}%
%	\fi%
%}
%\newcommand*\pdvm@star[2]{%
%	B%\abs{ #1 , #2 } \:
%%	\ifnum #2=2
%%		\pdvm@two{\pdvm@str@slsh}{#1}%
%%	\fi%
%}
%\newcommand*\pdvm@sstar[1]{%
%	C|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@flat}{}%
%	\fi%
%}
%
%\newcommand\pdvm@staropt[1][]{%
%	a| #1 | \:%
%	\if \relax\detokenize{#1}\relax
%		b%
%		\pdvm@star{}%
%	\else
%		c%
%		\pdvm@star{#1}%
%	\fi
%}
%\newcommand*\pdvm@STAR{\@ifstar{\pdvm@sstar}{\pdvm@staropt}}
%\newcommand*\pdvm{\@ifstar{\pdvm@STAR}{\pdvm@nostar}}



%---VECTOR CALCULUS---
%Uses similar syntax to the physics package.
%
%\grad{f}	Gradient operator
%\div{f}	Divergence operator
%\curl{f}	Curl operator

\let\divisionsymbol\div

\newcommand\grad[1]{\nabla #1}
\renewcommand\div[1]{\nabla \dotp #1}
\newcommand\curl[1]{\nabla \times #1}





%---ORDER NOTATION---

%If order is used with an empty argument then dont use parenthesis
\newcommand{\order@text}[1]{	
	\if\relax\detokenize{#1}\relax% #1 is empty
	\else% #1 is nonempty
		\ppar*{#1}%\qty(#1)
	\fi
}

%Big O
\newcommand{\order}[1]{
	\mathcal{O}\order@text{#1}
}

%Little O
\newcommand{\lorder}[1]{
  	\mathchoice
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \displaystyle
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \textstyle
    	{{\scriptscriptstyle\mathcal{O}}\order@text{#1}}% \scriptstyle
    	{\scalebox{.6}{${\scriptscriptstyle\mathcal{O}}\order@text{#1}$}}%\scriptscriptstyle
  	}

%Big Theta
\newcommand{\Torder}[1]{
	\mathit{\Theta}\order@text{#1}
}




%---ASSORTED---

%%Upright math text
%\DeclareMathAlphabet{\mathup}{OT1}{\familydefault}{m}{n}

%Have equation span full width of collumn (good for equations in lists)
\newcommand{\eqnwide}{\displayindent0pt \displaywidth\textwidth}

%Use as 10^\nth
\newcommand{\nth}{\text{th}}

%Defined to be equal to
\@ifundefined{eqdef}{\newcommand{\eqdef}{\vcentcolon =}}{}%{\stackrel{\mathrm{def}}{=}}

%Text style fraction
\newcommand{\textfrac}[2] {{\textstyle\frac{#1}{#2}}}

%Omitted dummy variable as a dot
\newcommand*\omitdummy{\mathchoice
	{\omitdummy@{\displaystyle}{0.6}}
	{\omitdummy@{\textstyle}{0.6}}
	{\omitdummy@{\scriptstyle}{0.7}}
	{\omitdummy@{\scriptscriptstyle}{0.8}}
}
\newcommand*\omitdummy@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}

%Degree symbol
\newcommand{\degree}{^{\circ}}



%---ENVIRONMENTS---

%Like cases but with as many collumns as you like

\newenvironment{multicasesnobrac}[1][1]{%
%No braces
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}
}
\newenvironment{multicases}[1][1]{%
%Left braced
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}\right.
}
\newenvironment{multicasesd}[1][1]{%
%Left braced with display style
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{>{\displaystyle}{r}@{}>{\displaystyle}{l}}}
}{
	\end{array}\right.
}




%---SIDE BY SIDE SUBEQUATIONS---

%Multiple labeled equations on same line
\newlength{\sbsse@Wl}	%Width of left equation
\newlength{\sbsse@Wm}	%Width of mid text
\newlength{\sbsse@Wr}	%Width of right equation
\newlength{\sbsse@Wt}	%Width of tag
\newlength{\sbsse@We}	%Remaining width on line
\newlength{\sbsse@Wd}	%Remaining width divided into pieces

%Two equations side by side
\newcommand\sidebysidesubequations[6]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    midtext
	% #5    right subequation
	% #6    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{\text{#4}}
	\def\sbsse@Er{#5}
	\def\sbsse@Et{(\ref*{#1}a,b)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space, and midtext if any
			\if\relax\detokenize{#4}\relax
				\setlength{\sbsse@Wd}{\sbsse@We/3}
				\hspace{\sbsse@Wd}
			\else
				\setlength{\sbsse@Wd}{\sbsse@We/4}
				\hspace{\sbsse@Wd}\sbsse@Em\hspace{\sbsse@Wd}
			\fi
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#6}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}

%Three equations side by side
\newcommand\sidebysidesubequationsT[7]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    mid subequation
	% #5	mid label
	% #6    right subequation
	% #7    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{#4}
	\def\sbsse@Er{#6}
	\def\sbsse@Et{(\ref*{#1}a,b,c)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	\setlength{\sbsse@Wd}{\sbsse@We/4}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space
			\hspace{\sbsse@Wd}
			%Mid equation and label
			\sbsse@Em\refstepcounter{equation}\ltx@label{{#5}}
			%Space
			\hspace{\sbsse@Wd}
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#7}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}




\makeatother
